Computations of HOMFLY homology

Khovanov--Rozansky's HOMFLY homology is determined for all prime knots with up to 11 crossings by direct computations.

==> tables/intro-targets.tex <==
\begin{tabular}{r|rrrrrrr}
$n \setminus l$	& $\leq 11$	& $12$ & $13$ & $14$ & $15$ & $16$ & $17$\\
\hline
$\leq 8$ & $\mathbf{35}$ \\
$9$ & $\mathbf{43}$ & $\mathbf{5}$ & & $\textbf{1}$ \\
$10$ & $\mathbf{126}$ & $\mathbf{31}$ & $\textbf{2}$ & $\textbf{6}$ \\
$11$ & $\mathbf{237}$ & $\mathbf{135}$ & $\textbf{74}$ & $81$ & $14$ & $9$ & $2$\\
\end{tabular}
\caption{Targets of computation\\ ($n$: crossing number, $l$: braid length)}
\label{table:targets}
\vspace{1em}
